Constrained Role Mining

Role Based Access Control (RBAC) is a very popular access control model, for long time investigated and widely deployed in the security architecture of different enterprises. To implement RBAC, roles have to be firstly identified within the considered organization. Usually the process of (automatically) defining the roles in a bottom up way, starting from the permissions assigned to each user, is called {\it role mining}. In literature, the role mining problem has been formally analyzed and several techniques have been proposed in order to obtain a set of valid roles. Recently, the problem of defining different kind of constraints on the number and the size of the roles included in the resulting role set has been addressed. In this paper we provide a formal definition of the role mining problem under the cardinality constraint, i.e. restricting the maximum number of permissions that can be included in a role. We discuss formally the computational complexity of the problem and propose a novel heuristic. Furthermore we present experimental results obtained after the application of the proposed heuristic on both real and synthetic datasets, and compare the resulting performance to previous proposals

==> conclusions.tex <==
\section{Conclusions}

The role mining process, usually, returns a role infrastructure on the basis of the relationships among users and permissions contained in the $\upa-m$ matrix. However, the definition of a role-set really reflecting the internal functionalities of the examined organization remains a challenging task.
%To improve the efficiency of the whole process and the practicality of the returned set of roles, it is necessary to     
The need for managing different kind of constraints in role engineering has recently been the focus of many works in literature \cite{kumar10, HinSur11, MaLiLuWa11}. The definition and the management of constraints in role mining  are very important aspects in role mining, since they allow the role engineer to control the automatic process and introduce some rules that can have impact on the retrieved structure. 
In this paper, we have proposed a heuristic capable of returning a complete role-set satisfying constraints on the maximum number of permissions included in each role. The comparisons made show how the results in terms of accuracy, distance, size, and computation time improve on a previously presented algorithm \cite{kumar10}. 
Our simple algorithm is easily extensible to consider other kinds of cardinality constraints, such as maximum number of users assigned to a role or mutually exclusive permissions or roles \cite{MaLiLuWa11}. 
Furthermore, it is possible to investigate on the definition of other kinds of constraints regarding the role hierarchy and the semantic associated to each role \cite{semantic08}, and try  to adapt the proposed algorithm in order to return a role set satisfying the newly defined constraints.   
\label{conclusions}


==> introduction.tex <==
\section{Introduction}

Complex organizations need to establish access control policies in order
to manage access to restricted resources. A simple way to accomplish this
task is to collect set of permissions in roles and then assign roles 
according to the responsibilities and qualifications of each employee. 
The Role Based Access Control (RBAC) is a well known paradigm to define and
organize roles and permissions in an efficient way. Introduced in the 
  early '90 years \cite{coyne,nist},such a paradigm has been
 investigated for long time and has become recently used in different
 commercial systems to manage identities and accounts \cite{ibmtivoli}.
The goal of RBAC is to collect set of permissions in roles and define a complete 
and efficient set of roles that can be assigned to users in order 
to access restricted resources.
The advantage is that access control can
be centralized and decoupled from users and  the costs and the  overhead of
the security management can be reduced. 


The correct definition of the set of roles which satisfies the needs of the
organization is  the most difficult and costly task to be performed during
the implementation of  a RBAC system. Such an activity is often referred to
as {\it role engineering} and includes 
the correct identification of roles from the current structural
organization of the enterprise. 
Mainly this task, i.e. the extraction of a complete and
efficient set of roles, can be performed using two approaches: 
\emph{top-down} or \emph{bottom-up} role
engineering. In the first case, roles are defined after that the
functionalities of the organization have been well defined and studied, and
elicitation activities have been performed. 
The top down approach usually is labor intensive and 
involves a large amount of work and time done by humans especially in large
enterprises with a large number of business processes, as reported in  some case study are
available in the literature \cite{Roeckle00}. 
On the other hand, the bottom-up process, often denoted also as \emph{role mining}
starts from  the analysis of the current set of permissions assigned to
users, and tries to aggregate them in order to extract and define roles. 
Obviously, hybrid approaches can exist
in which both directions, top-down and bottom-up, can be used in subsequent
steps of the analysis in order to refine the returned set of roles. 

Bottom-up approach to role mining has been more investigated, since many 
techniques borrowed from data mining can be applied in an automatic way to
the existing configuration of user-permission assignments. 
A RBAC system can be easily constructed in this way and a starting set of roles can 
be fastly generated. The problem with such an approach, is that the quality and the 
number of returned roles often are not so good, since no semantics is taken into consideration when
the role mining process is started. In many situations the returned set of roles might
not match any functional organization within the analyzed enterprise and the
existing business processes might not be adequately represented.  An
accurate analysis of the returned results is needed to better tune the
retrieved representation of roles to the current organizational requirements of 
the  enterprise.
A formal definition of the  Role
Mining Problem (RMP) and some of its variants  has been given and deeply analyzed in 
\cite{sacmat07}. There, the NP-completeness of the (decisional) 
RMP problem has been proved, and the formulation of RMP as a graph covering
problem has been done in \cite{biclique,zhang07}.


The problem of imposing constraints on the set of roles resulting after the
role mining process has been considered in the past. Statically or
dynamically mutually exclusive roles constraints have been included in RBAC
models \cite{Sandhu96} and in the NASI/NIST standards \cite{nist}. According to these
constraints, for examples, no user can be assigned contemporary a given set
of mutually exclusive roles, or no user can activate simultaneously a set of
roles in the same session. Such constraints are often used as mechanisms 
to achieve separation of duty principles, preventing one user from having a
large number of roles to complete a task, or imposing restrictions on the
minimum number of users needed to perform a critical activity \cite{Li2007}.


Recently, a simple classification of the constraints on the cardinality of
the number of roles, users and permissions for a given RBAC system has been
proposed \cite{MaLiLuWa11}. The first heuristic taking into account a
cardinality constraint on the number of permissions contained in a role has
been proposed by \cite{kumar10}. In its work, however, the proposed results
have been compared only on other heuristics which were not able to consider
constrained roles.
In this work we propose a novel heuristic for mining RBAC roles under
cardinality constraint. The algorithm is based on  a previous 
proposal \cite{sac10}, where  an initial candidate role set was constructed by
considering one role for each user on the basis of the current assignment 
of permissions. The role set is then refined and updated by eliminating the 
roles obtained as union of other roles already included in the set and
ensuring that the cardinality constraint is respected. Finally, an optimization of
the role set is performed by running a lattice reduction procedure,
previously described in \cite{biclique}.
The resulting procedure is very efficient in terms of computation time and
quality of returned role set.
To this aim we present
the results obtained by running our heuristics on different datasets, some
available over the network, some artificially created. The results are
compared with our implementation of the algorithm presented in \cite{kumar10}
and analyzed in terms of the metrics presented in \cite{MolloyLLMWL09}.

The remainder of this paper is organized as follows. In the next section we
discuss related works. Section \ref{np} contains the preliminary concepts needed to
define the constrained role mining problem and the discussion on its
complexity. In section \ref{ksma} we introduce our heuristics and compare the solution with related
work in section \ref{experiments}. Finally Section \ref{conclusions} presents our conclusions and
ongoing work.



==> related.tex <==
\section{Related Works}
\label{related}
Role engineering has been firstly introduced by Coyne et al in \cite{coyne} where the definition of a top down process for the definition of roles   
has been discussed. 
%Along the same research line, several other works have been presented \cite{Fer97, Roeckle00, Neu02}, 
Along the same research line, several other works have been presented \cite{Roeckle00}, 
but recently, the focus of role engineering has turned to consider more automated techniques, based on the bottom up approach,  where data mining techniques are applied for the definition of roles \cite{Kuh03}. Role mining algorithms have been presented based on set covering  \cite{ChCr09}, graph theory \cite{biclique, zhang07}, subset enumeration \cite{ccs06}, database tiling \cite{sacmat07}. 
The theoretical aspects of the RMP have been considered in \cite{VaidyaAG10,sacmat07,ChCr09}, where the complexity of the problem has been analyzed and its equivalence to other known optimization problem showed. Another interrelated  problem, i.e. dealing with the semantic meaning of roles, has been addressed in \cite{semantic08}. 

Cardinality constraints on the number of permissions included in a role  have been firstly considered in \cite{kumar10}, and a heuristic algorithm called Constrained Role Miner (CRM) has been proposed. The CRM algorithm takes in input the \up\ matrix and returns a set of roles, each one satisfying the given cardinality constraint. CRM is based on the idea of clustering users having the same set of permissions and selecting, as candidate roles, the roles composed of the set of permissions satisfying the constraint  and having the highest number of associated users.
 In \cite{kumar10}, the performances of the algorithm are evaluated on real world datasets considering different metrics (such as the number of returned roles, the sum of the size of the user assignment and permission assignment matrices and so on), with respect to other previously proposed algorithms. However the comparison is performed without  considering constraints,  since the other algorithms return a complete set of roles but have not the capability of managing constraints. In section \ref{experiments} we evaluate our proposal against the result obtained after our implementation of the CRM algorithm, considering both real world and synthetic datasets.
A different kind of cardinality constraints, considering the number of user-role assignments, have been considered in \cite{HinSur11}. Such constraints can be useful when the number of persons that can be assigned to a given role (e.g. the number of directors, managers, etc) in a given organization is known or can be fixed. In the paper, three algorithms have been proposed based on a graph approach, where the role mining problem is mapped to the problem of finding minimum biclique cover of the edges of a bipartite graph. The three heuristics are obtained by modifying the basic greedy algorithm proposed in \cite{biclique}, and experimental results on real world datasets  are reported considering some constraints on the number of users that can be assigned to any role.
Finally cardinality constraints have also been considered in \cite{MaLiLuWa11} where a representation of the constraints in terms of association rules is proposed: permissions are regarded as attributes, and each user-permission assignment as a transaction. To generate mutually exclusive permissions constraints, i.e. set of permissions that cannot be assigned to the same role, an algorithm is proposed, based on known techniques for mining association rules in databases, and its performance evaluated on synthetically generated datasets
 
